Systematic KMTNet Planetary Anomaly Search. XII. Complete Sample of 2017 Subprime Field Planets

We report the analysis of four unambiguous planets and one possible planet from the subprime fields ($\Gamma \leq 1~{\rm hr}^{-1}$) of the 2017 Korea Microlensing Telescope Network (KMTNet) microlensing survey, to complete the KMTNet AnomalyFinder planetary sample for the 2017 subprime fields. They are KMT-2017-BLG-0849, KMT-2017-BLG-1057, OGLE-2017-BLG-0364, and KMT-2017-BLG-2331 (unambiguous), as well as KMT-2017-BLG-0958 (possible). For the four unambiguous planets, the mean planet-host mass ratios, $q$, are $(1.0, 1.2, 4.6, 13) \times 10^{-4}$, the median planetary masses are $(6.4, 24, 76, 171)~M_{\oplus}$ and the median host masses are $(0.19, 0.57, 0.49, 0.40)~M_{\odot}$ from a Bayesian analysis. We have completed the AnomalyFinder planetary sample from the first 4-year KMTNet data (2016--2019), with 112 unambiguous planets in total, which nearly tripled the microlensing planetary sample. The ``sub-Saturn desert'' ($\log q = \left[-3.6, -3.0\right]$) found in the 2018 and 2019 KMTNet samples is confirmed by the 2016 and 2017 KMTNet samples.

==> backup.tex <==


\subsection{\evente}

\begin{figure}[htb] 
    \centering
    \includegraphics[width=0.95\columnwidth]{Figure/KB171237-lc.pdf}
    \caption{Observed data and the four 2L1S models for \evente.}
    \label{lc-e}
\end{figure}

\begin{figure*}[htb] 
    \centering
    \includegraphics[width=0.75\textwidth]{Figure/cau_kb171237.pdf}
    \caption{Caustic geometries of the four models of \evente.}
    \label{cau-e}
\end{figure*}

\begin{table*}[htb]
    \renewcommand\arraystretch{1.25}
    \centering
    \caption{2L1S Parameters for \evente}
    \begin{tabular}{c|c|c|c|c}
    \hline
    \hline
    Parameters & \multicolumn{2}{c|}{A} & \multicolumn{2}{c}{B} \\
    \hline
    & Wide & Close & Wide & Close\\
    \hline
    $\chi^2$/dof & $1666.09/1666$ & $1666.52/1666$& $1968.23/1666$& $1957.13/1666$\\
    \hline
    $t_{0}$ (${\rm HJD}^{\prime}$)  & $8000.984\pm0.001$& $8000.974\pm0.001$& $7999.02\pm0.11$& $8000.982\pm0.002$\\
    $u_{0}$  & $0.0234\pm 0.0004$ & $0.0135\pm0.0001$& $0.042\pm0.003$ & $0.0140\pm 0.0001$\\
    $\te$ (days)  & $23.26\pm0.23$ & $23.22\pm0.18$& $23.00\pm0.22$ & $22.58\pm0.18$\\
    $\rho$ ($10^{-3}$) & $<4.6$ & $<4.5$& $<2.4$ & $<2.0$\\
    $\alpha$ (rad) & $1.527\pm0.004$ & $1.528\pm0.005$& $2.565\pm0.003$ & $3.721\pm0.003$\\
    $s$ & $1.84\pm 0.02$ & $0.54\pm0.01$& $3.57\pm0.06$ & $0.29\pm0.01$\\
    $q (10^{-3})$ & $7.68\pm0.15$ & $7.60\pm0.14$& $32.00\pm1.28$ & $31.07\pm1.53$\\
    $\log q$ & $-2.114\pm0.009$ & $-2.119\pm0.008$& $-1.495\pm0.018$ & $-1.508\pm0.021$\\
    $f_{\rm S, OGLE}$ & $0.533\pm0.006$ & $0.531\pm0.005$& $0.550\pm0.006$ & $0.551\pm0.005$\\
    $f_{\rm B, OGLE}$ & $0.183\pm0.006$ & $0.184\pm0.005$& $0.167\pm0.006$ & $0.165\pm0.005$\\
    \hline
    \hline
    \end{tabular}
    \label{parm-e}
     % sigma(piee) ~ 0.1
\end{table*}

As shown Figure \ref{lc-e}, the anomaly of \evente\ is a 3-bump feature on a high-magnification PSPL peak, which could be caused by three cusps of a central caustic, respectively, and the source trajectory roughly perpendicular to the planet-host axis on the opposite side of the planet. A finite-source/point-lens (FSPL) model cannot fit the anomaly. A 2L1S grid search yields two pairs of models, and each pair is subject to the so-called close-wide degeneracy \citep{Griest1998, Dominik1999}. 



For wide/close A solutions, the geometric mean of the two solutions (0.996) is close to unity (the close-wide prediction). For this event, another pair of wide/close degeneracy solutions are shown in Table  but are basically disfavored by $\mathrm{\Delta}\chi^2>300$.



\subsection{\eventf}
Figure \ref{lc-f} shows a pronounced long $(\sim 10\ {\rm days})$ bump centered at $t_{\rm anom}\sim7845$ before the peak of a normal 1L1S event with parameters $t_0 = 7852.9$, $u_0 = 0.011$, and $t_{\rm E} = 93.52$ days, so we obtain $\tau_{\rm anom} = -0.084$, $u_{\rm anom} = 0.085$, $\alpha = 191.3^\circ$, and $s_+ \sim 1.04$ or $s_- \sim 1.04$. 

The grid search returns two local minima, whose refinements are shown in Table \ref{parm-f} and that are in good agreement with these predictions, i.e., $s^\dag=\sqrt{s_{\rm close}s_{\rm wide}}=1.01$, and $\alpha = 191.2^\circ$.

Because the event is moderately long, the source is relatively bright and the photometry is good, we attempt to measure $\pie$. 

Figure \ref{cau-f} shows 2L1S wide/close caustic crossing geometries.

We also check 1L2S model. Table \ref{parm-f-2} shows 1L2S best-fit parameters. Because $\Delta \chi^2 >45$, they are excluded compared to the wide best-fit model.

\begin{figure}[htb] 
    \centering
    \includegraphics[width=0.95\columnwidth]{Figure/KB171136-lc.pdf}
    \caption{Observed data and the 2L1S and 1L2S for \eventf. The symbols are similar to those in Figure \ref{lc-a-total}.}
    \label{lc-f}
\end{figure}

\begin{figure}[htb] 
    \centering
    \includegraphics[width=0.95\columnwidth]{Figure/cau_kb171136.pdf}
    \caption{Caustic crossing geometries of \eventf\ models. The symbols are similar to those in Figure \ref{cau-a}.}
    \label{cau-f}
\end{figure}


    \hline
    \evente & 28 Aug 2017 & 18:09:31.86 & $-$27:43:20.9 & +3.6853 & $-$3.9487 & 1--3 per night \\
    MOA-2017-BLG-441 & & & & & & $1.2~{\rm hr}^{-1}$ \\
    KMT-2017-BLG-1237 & & & & & & $0.4~{\rm hr}^{-1}$ \\
    \hline
    \eventf & 12 Mar 2017 & 17:58:51.94 & $-$32:26:59.8 & $-$1.5800 & $-$4.2376 & 1--3 per night \\
    MOA-2017-BLG-441 & & & & & & $1.2~{\rm hr}^{-1}$ \\
    KMT-2017-BLG-1237 & & & & & & $1.0~{\rm hr}^{-1}$ \\




\author{Takahiro Sumi}
\affiliation{Department of Earth and Space Science, Graduate School of Science, Osaka University, Toyonaka, Osaka 560-0043, Japan}

\author{Fumio Abe}
\affiliation{Institute for Space-Earth Environmental Research, Nagoya University, Nagoya 464-8601, Japan}
%abe@isee.nagoya-u.ac.jp

\author{Richard Barry}
\affiliation{Code 667, NASA Goddard Space Flight Center, Greenbelt, MD 20771, USA}
%richard.k.barry@nasa.gov

\author{David P. Bennett}
\affiliation{Code 667, NASA Goddard Space Flight Center, Greenbelt, MD 20771, USA}
\affiliation{Department of Astronomy, University of Maryland, College Park, MD 20742, USA}
%david.p.bennett@nasa.gov

\author{Aparna Bhattacharya}
\affiliation{Code 667, NASA Goddard Space Flight Center, Greenbelt, MD 20771, USA}
\affiliation{Department of Astronomy, University of Maryland, College Park, MD 20742, USA}
%abhatta5@umd.edu

\author{Ian A. Bond}
\affiliation{Institute of Natural and Mathematical Sciences, Massey University, Auckland 0745, New Zealand}
%I.A.Bond@massey.ac.nz

\author{Hirosane Fujii}
\affiliation{Department of Earth and Space Science, Graduate School of Science, Osaka University, Toyonaka, Osaka 560-0043, Japan}
%hfuji@iral.ess.sci.osaka-u.ac.jp

\author{Akihiko Fukui}
\affiliation{Department of Earth and Planetary Science, Graduate School of Science, The University of Tokyo, 7-3-1 Hongo, Bunkyo-ku, Tokyo 113-0033, Japan}
\affiliation{Instituto de Astrof\'isica de Canarias, V\'ia L\'actea s/n, E-38205 La Laguna, Tenerife, Spain}
%afukui@eps.s.u-tokyo.ac.jp

\author{Ryusei Hamada}
\affiliation{Department of Earth and Space Science, Graduate School of Science, Osaka University, Toyonaka, Osaka 560-0043, Japan}

\author{Yuki Hirao}
\affiliation{Department of Earth and Space Science, Graduate School of Science, Osaka University, Toyonaka, Osaka 560-0043, Japan}
%hirao@iral.ess.sci.osaka-u.ac.jp

\author{Stela Ishitani Silva}
\affiliation{Department of Physics, The Catholic University of America, Washington, DC 20064, USA}
\affiliation{Code 667, NASA Goddard Space Flight Center, Greenbelt, MD 20771, USA}
%StelaIS@gmail.com

\author{Yoshitaka Itow}
\affiliation{Institute for Space-Earth Environmental Research, Nagoya University, Nagoya 464-8601, Japan}
%itow@isee.nagoya-u.ac.jp

\author{Rintaro Kirikawa}
\affiliation{Department of Earth and Space Science, Graduate School of Science, Osaka University, Toyonaka, Osaka 560-0043, Japan}
%kirikawa@iral.ess.sci.osaka-u.ac.jp

\author{Iona Kondo}
\affiliation{Department of Earth and Space Science, Graduate School of Science, Osaka University, Toyonaka, Osaka 560-0043, Japan}
%ikondoh@iral.ess.sci.osaka-u.ac.jp

\author{Naoki Koshimoto}
\affiliation{Code 667, NASA Goddard Space Flight Center, Greenbelt, MD 20771, USA}
\affiliation{Department of Astronomy, University of Maryland, College Park, MD 20742, USA}
%koshimoto@astron.s.u-tokyo.ac.jp

\author{Yutaka Matsubara}
\affiliation{Institute for Space-Earth Environmental Research, Nagoya University, Nagoya 464-8601, Japan}
%ymatsu@isee.nagoya-u.ac.jp

\author{Sho Matsumoto}
\affiliation{Department of Earth and Space Science, Graduate School of Science, Osaka University, Toyonaka, Osaka 560-0043, Japan}

\author{Shota Miyazaki}
\affiliation{Department of Earth and Space Science, Graduate School of Science, Osaka University, Toyonaka, Osaka 560-0043, Japan}
%miyazaki@iral.ess.sci.osaka-u.ac.jp

\author{Yasushi Muraki}
\affiliation{Institute for Space-Earth Environmental Research, Nagoya University, Nagoya 464-8601, Japan}
%ysa_muraki@topaz.plala.or.jp

\author{Arisa Okamura}
\affiliation{Department of Earth and Space Science, Graduate School of Science, Osaka University, Toyonaka, Osaka 560-0043, Japan}

\author{Greg Olmschenk}
\affiliation{Code 667, NASA Goddard Space Flight Center, Greenbelt, MD 20771, USA}
%golmschenk@usra.edu

\author{Cl\'ement Ranc}
\affiliation{Sorbonne Universit\'e, CNRS, Institut d'Astrophysique de Paris, IAP, F-75014, Paris, France}
%clement.ranc@protonmail.com

\author{Nicholas J. Rattenbury}
\affiliation{Department of Physics, University of Auckland, Private Bag 92019, Auckland, New Zealand}
%n.rattenbury@auckland.ac.nz

\author{Yuki Satoh}
\affiliation{Department of Earth and Space Science, Graduate School of Science, Osaka University, Toyonaka, Osaka 560-0043, Japan}
%satohyk@iral.ess.sci.osaka-u.ac.jp

\author{Daisuke Suzuki}
\affiliation{Department of Earth and Space Science, Graduate School of Science, Osaka University, Toyonaka, Osaka 560-0043, Japan}

\author{Taiga Toda}
\affiliation{Department of Earth and Space Science, Graduate School of Science, Osaka University, Toyonaka, Osaka 560-0043, Japan}

\author{Mio Tomoyoshi}
\affiliation{Department of Earth and Space Science, Graduate School of Science, Osaka University, Toyonaka, Osaka 560-0043, Japan}

\author{Paul J. Tristram}
\affiliation{University of Canterbury Mt.\ John Observatory, P.O. Box 56, Lake Tekapo 8770, New Zealand}
%tristram.p@gmail.com

\author{Aikaterini Vandorou}
\affiliation{Code 667, NASA Goddard Space Flight Center, Greenbelt, MD 20771, USA}
\affiliation{Department of Astronomy, University of Maryland, College Park, MD 20742, USA}

\author{Hibiki Yama}
\affiliation{Department of Earth and Space Science, Graduate School of Science, Osaka University, Toyonaka, Osaka 560-0043, Japan}

\author{Kansuke Yamashita}
\affiliation{Department of Earth and Space Science, Graduate School of Science, Osaka University, Toyonaka, Osaka 560-0043, Japan}

\collaboration{(The MOA Collaboration)}


and the Microlensing Observations in Astrophysics (MOA) group observed using one 1.8 m telescope equipped with 2.2 ${\rm deg}^2$ camera in New Zealand \citep{Sako2008}.

\begin{table*}[htb]
    \renewcommand\arraystretch{1.25}
    \centering
    \caption{2L1S Parameters for \eventf}
    \begin{tabular}{c|c|c|c|c|c|c}
    \hline
    \hline
    \multirow{2}{*}{Parameters} & \multicolumn{2}{c|}{Wide A} & \multicolumn{2}{c|}{Wide B} &\multicolumn{2}{c}{Close}\\
    \cline{2-7}
    & $u_0>0$ & $u_0<0$& $u_0>0$ & $u_0<0$  & $u_0>0$ &$u_0<0$\\
    \hline
    $\chi^2$/dof & $2188.06/2188$ & $2191.92/2188$ &  $2231.04/2188$ &$2229.93/2188$ &$2235.21/2188$ &$2231.52/2188$\\
    \hline
    $t_{0}$ (${\rm HJD}^{\prime}$)  & $7852.17\pm0.09$ & $7852.08\pm0.11$ & $7852.78\pm0.02$ & $7852.77\pm0.02$ & $7852.57\pm0.01$ & $7852.56\pm0.01$ \\
    $u_{0}$  & $0.011\pm 0.001$& $-0.011\pm 0.001$& $0.010\pm 0.001$ &$-0.011\pm0.001$ & $0.016\pm 0.001$ & $-0.017\pm 0.001$ \\
    $\te$ (days)  & $117.12\pm5.82$ & $112.62\pm6.37$  & $119.27\pm7.72$ &$113.84\pm7.35$ & $85.60\pm4.48$ & $83.51\pm3.95$  \\
    $\rho$ ($10^{-3}$) & $5.88\pm0.48$ & $6.76\pm0.69$ & $8.52\pm0.53$ & $8.93\pm0.54$ & $9.24\pm0.69$ & $9.53\pm0.73$ \\
    $\alpha$ (rad) & $3.34\pm0.02$ & $-3.33\pm0.02$ & $3.11\pm0.01$ & $-3.11\pm0.01$ & $3.24\pm0.01$ & $-3.24\pm0.003$ \\
    $s$ & $1.367\pm 0.024$ & $1.414\pm 0.037$ & $1.31\pm 0.01$ & $1.32\pm0.01$ & $0.744\pm0.009$ & $0.741\pm0.010$ \\
    $q (10^{-3})$  & $5.22\pm0.52$ & $6.39\pm0.91$ & $1.85\pm0.21$ & $1.98\pm0.22$ & $6.14\pm0.82$ &$6.51\pm0.96$\\
    $\log q$ &  $-2.285\pm0.042$ &  $-2.199\pm0.061$ & $-2.736\pm0.050$ &$-2.705\pm0.049$ & $-2.216\pm0.058$ & $-2.191\pm0.063$ \\
    $\pi_{\rm E,N}$  & $-0.725\pm0.077$ &$0.796\pm0.171$  & $0.978\pm0.057$& $-1.008\pm0.065$ &$-0.074\pm0.038$ & $0.118\pm0.033$ \\
    $\pi_{\rm E,E}$  &$-0.416\pm0.033$ & $-0.358\pm0.044$& $-0.335\pm0.023$& $-0.458\pm0.031$ &$-0.110\pm0.034$ &$-0.109\pm0.023$ \\
    $f_{\rm S, OGLE}$ &$0.043\pm0.002$  &$0.045\pm0.003$  & $0.043\pm0.003$ & $0.046\pm0.003$ & $0.063\pm0.004$ & $0.064\pm0.004$ \\
    $f_{\rm B, OGLE}$ & $0.371\pm0.002$&$0.371\pm0.003$ & $0.373\pm 0.002$ & $0.368\pm0.002$ & $0.348\pm 0.003$ & $0.346\pm0.003$ \\
    \hline
    \hline
    \end{tabular}
    \tablecomments{All fluxes are on an 18th magnitude scale, e.g., $I_{\rm S} = 18 - 2.5 \log(f_{\rm S})$.}
    \label{parm-f}
\end{table*}

\begin{table*}[htb]
    \renewcommand\arraystretch{1.25}
    \centering
    \caption{1L2S Parameters for \eventf}
    \begin{tabular}{c|c|c}
    \hline
    \hline
    \multirow{2}{*}{Parameters} & \multicolumn{2}{c}{1L2S}\\
    \cline{2-3}
    & $u_0>0$ & $u_0<0$\\
    \hline
    $\chi^2$/dof & $2235.49/2187$ & $2234.78/2187$ \\
    \hline
    $t_{0,1}$ (${\rm HJD}^{\prime}$)  & $7853.08\pm0.01$ & $7853.08\pm0.01$ \\
    $t_{0,2}$ (${\rm HJD}^{\prime}$)  & $7845.58\pm 0.17$ &$7845.75\pm0.21$ \\
    $u_{0,1}$  & $0.012\pm0.001$ & $-0.0115\pm0.0004$ \\
    $u_{0,2}$  & $0.030\pm 0.005$ &$-0.0320\pm0.0004$ \\
    $\te$ (days)  & $76.00\pm4.34$ &$77.04\pm2.63$ \\
    $\rho_2$ ($10^{-2}$) & $<3.3$ & $<2.9$ \\
    $q_{f,I}$ & $0.172\pm0.011$ & $0.166\pm0.011$ \\
    $q_{f,V}$ & $0.096\pm0.021$ & $0.093\pm0.020$ \\
    $\pi_{\rm E,N}$ & $-0.454\pm0.358$& $-0.025\pm0.482$\\
    $\pi_{\rm E,E}$ & $-0.323\pm0.034$& $-0.304\pm0.032$\\
    $f_{\rm S, OGLE}$ & $0.070\pm0.004$ & $0.069\pm0.003$\\
    $f_{\rm B, OGLE}$ & $0.343\pm0.004$ & $0.345\pm0.003$\\
    \hline
    \hline
    \end{tabular}
    \tablecomments{All fluxes are on an 18th magnitude scale, e.g., $I_{\rm S} = 18 - 2.5 \log(f_{\rm S})$.}
    \label{parm-f-2}
\end{table*}


\begin{table*}[htb]
    \renewcommand\arraystretch{1.25}
    \centering
    \caption{CMD Parameters, $\theta_\ast$, $\theta_{\rm E}$, and $\mu_{\rm rel}$ for \eventf}
    \begin{tabular}{c| c c c c c c}
    \hline
    \hline
    Parameter & \multicolumn{2}{c}{Wide A}& \multicolumn{2}{c}{Wide B}&\multicolumn{2}{c}{Close}\\
    \cline{2-7}
     &  $u_0>0$&$u_0<0$&   $u_0>0$&$u_0<0$& $u_0>0$&$u_0<0$\\
    \hline
    $(V-I)_{\rm cl}$ & $2.02\pm0.01$ &$\longleftarrow$  & $\longleftarrow$   &$\longleftarrow$   &$ \longleftarrow$  &$ \longleftarrow$  \\
    $I_{\rm cl}$ & $15.61\pm0.05$ &$\longleftarrow$  & $\longleftarrow$   &$\longleftarrow$   &$\longleftarrow $ &$\longleftarrow $ \\
    $(V-I)_{\rm cl.0}$ & $1.06\pm0.03$  &$\longleftarrow$  & $\longleftarrow$   &$\longleftarrow$   &$\longleftarrow$  &$\longleftarrow$  \\
    $I_{\rm cl,0}$ & $14.53\pm0.04$ &$\longleftarrow$  & $\longleftarrow$   &$\longleftarrow$   &$\longleftarrow$  &$\longleftarrow$  \\
    $(V-I)_{\rm S}$ & $1.87\pm0.01$ &$\longleftarrow$  & $\longleftarrow$   &$\longleftarrow$   &$\longleftarrow$  &$\longleftarrow$  \\
    $I_{\rm S}$ & $21.43\pm0.06$&$21.38\pm0.07$& $21.42\pm0.07$&$21.34\pm0.07$&$21.01\pm0.07$&$20.98\pm0.07$\\
    $(V-I)_{\rm S,0}$ & $0.90\pm0.04$ &$\longleftarrow$ & $\longleftarrow$  &$\longleftarrow$  &$\longleftarrow$ &$\longleftarrow$ \\
    $I_{\rm S,0}$ & $20.35\pm0.09$&$20.30\pm0.10$& $20.34\pm0.10$&$20.26\pm0.10$&$19.93\pm0.10$&$19.90\pm0.10$\\
    $\theta_\ast$ ($\mu$as)& $0.325\pm0.017$&$0.333\pm0.018$& $0.327\pm0.018$&$0.338\pm0.019$&$0.395\pm0.021$&$0.400\pm0.022$\\
    $\theta_{\rm E}$ (mas)& $0.055\pm0.005$&$0.049\pm0.006$& $0.038\pm0.003$&$0.037\pm0.003$&$0.043\pm0.004$&$0.042\pm0.004$\\
    $\mu_{\rm rel}$ (mas $\mathrm{yr}^{-1}$)& $0.17\pm0.02$&$0.16\pm0.02$& $0.12\pm0.01$&$0.12\pm0.01$&$0.18\pm0.02$&$0.18\pm0.02$\\
    \hline
    \end{tabular}
    %\tablecomments{$P_\mathrm{{bulge}}$ is the probability that the lens is in the Galactic bulge.}
    \label{lens2}
\end{table*}


\begin{figure*}[htb] 
    \centering
    \includegraphics[width=0.8\textwidth]{Figure/KB170849_publish_figure_bayes.pdf}
    \includegraphics[width=0.8\textwidth]{Figure/OB170364_publish_figure_bayes.pdf}
    \caption{Bayesian posterior distributions of the mass of the host star, $M_\mathrm{host}$, the planetary mass, $M_\mathrm{planet}$, the lens distance, $D_\mathrm{L}$, the projected planet-host separation, $r_\bot$, and the lens-source relative proper motion in the heliocentric frame, $\mu_\mathrm{hel, rel}$. In each panel, the solid black line and the two dashed black lines represent the median value and the 15.9\% and 84.1\% percentages of the distribution, and the corresponding values are presented in Table \ref{baysparm}. The solid black histogram shows the total distribution, and the bulge and disk lens distributions are shown in red and blue, respectively.}
    \label{baysfigure}
\end{figure*}

==> figure.tex <==








==> table.tex <==










\begin{table*}[htb]
    \renewcommand\arraystretch{1.25}
    \centering
    \caption{CMD Parameters, $\theta_\ast$, $\theta_{\rm E}$, and $\mu_{\rm rel}$ for Two Events}
    \begin{tabular}{c c c}
    \hline
    \hline
    Parameter & \eventb & \eventd\\
    \hline
    $(V-I)_{\rm cl}$ & $2.25\pm0.01$ & $3.59\pm0.03$ \\
    $I_{\rm cl}$ & $15.63\pm0.07$ &  $17.91\pm0.07$ \\
    $(V-I)_{\rm cl.0}$ & $1.06\pm0.03$ & $1.06\pm0.03$ \\
    $I_{\rm cl,0}$ & $14.30\pm0.04$&  $14.52\pm0.04$   \\
    $(V-I)_{\rm S}$ & $2.14\pm0.17$ & $3.29\pm0.13$  \\
    $I_{\rm S}$ & $20.78\pm0.07$&  $22.63\pm0.09$\\
    $(V-I)_{\rm S,0}$ & $0.95\pm0.17$ & $0.77\pm0.14$ \\
    $I_{\rm S,0}$ & $19.45\pm0.11$& $19.25\pm0.12$\\
    $\theta_\ast$ ($\mu$as)& $0.512\pm0.080$& $0.482\pm0.064$\\
    $\theta_{\rm E}$ (mas)& $>0.233$& $0.233\pm0.046$\\
    $\mu_{\rm rel}$ (mas $\mathrm{yr}^{-1}$)& $>2.80$& $1.77\pm0.37$\\
    \hline
    \end{tabular}
    \tablecomments{Event names are abbreviations, e.g., KMT-2017-BLG-1057 to KB171057.}
    \label{lens1}
\end{table*}


\begin{table*}[htb]
    \renewcommand\arraystretch{1.25}
    \centering
    \caption{CMD Parameters, $\theta_\ast$, $\theta_{\rm E}$, and $\mu_{\rm rel}$ for \eventg}
    \begin{tabular}{c| c c c c}
    \hline
    \hline
    Parameter & Wide A & Close A & Wide B & Close B\\
    \hline
    $(V-I)_{\rm cl}$ & $1.82\pm0.01$ &$ \longleftarrow$ & $\longleftarrow$ & $\longleftarrow$ \\
    $I_{\rm cl}$ & $15.29\pm0.05$ & $\longleftarrow $& $\longleftarrow$ & $\longleftarrow$ \\
    $(V-I)_{\rm cl.0}$ & $1.06\pm0.03$ & $\longleftarrow$ & $\longleftarrow$ & $\longleftarrow$ \\
    $I_{\rm cl,0}$ & $14.34\pm0.04$& $\longleftarrow$ & $\longleftarrow$ & $\longleftarrow$ \\
    $(V-I)_{\rm S}$ & $1.58\pm0.01$ & $\longleftarrow$ & $\longleftarrow$ & $\longleftarrow$ \\
    $I_{\rm S}$ & $18.74\pm0.01$& $18.73\pm0.01$& $18.70\pm0.01$& $18.69\pm0.01$\\
    $(V-I)_{\rm S,0}$ & $0.82\pm0.03$ & $\longleftarrow$& $\longleftarrow$& $\longleftarrow$\\
    $I_{\rm S,0}$ & $17.78\pm0.06$& $17.77\pm0.06$& $17.74\pm0.06$& $17.74\pm0.06$\\
    $\theta_\ast$ ($\mu$as)& $0.989\pm0.039$& $0.993\pm0.040$& $1.007\pm0.040$& $1.009\pm0.040$\\
    $\theta_{\rm E}$ (mas)& $>0.206$& $>0.236$& $>0.387$& $>0.374$\\
    $\mu_{\rm rel}$ (mas $\mathrm{yr}^{-1}$)& $>3.25$& $>3.74$& $>6.15$& $>5.92$\\
    \hline
    \end{tabular}
    %\tablecomments{$P_\mathrm{{bulge}}$ is the probability that the lens is in the Galactic bulge.}
    \label{lens3}
\end{table*}

\begin{table*}[htb]
    \renewcommand\arraystretch{1.25}
    \centering
    \caption{CMD Parameters, $\theta_\ast$, $\theta_{\rm E}$, and $\mu_{\rm rel}$ for \eventa}
    \begin{tabular}{c c c c c}
    \hline
    \hline
    Parameter & Wide A & Wide B & Wide C & Wide D\\
    \hline
    $(V-I)_{\rm cl}$ & $3.02\pm0.01$ &$ \longleftarrow$ & $\longleftarrow$ & $\longleftarrow$ \\
    $I_{\rm cl}$ & $16.72\pm0.04$ & $\longleftarrow $& $\longleftarrow$ & $\longleftarrow$ \\
    $(V-I)_{\rm cl.0}$ & $1.06\pm0.03$ & $\longleftarrow$ & $\longleftarrow$ & $\longleftarrow$ \\
    $I_{\rm cl,0}$ & $14.30\pm0.04$& $\longleftarrow$ & $\longleftarrow$ & $\longleftarrow$ \\
    $(V-I)_{\rm S}$ & $2.99\pm0.10$ & $2.92\pm0.09$ & $2.92\pm0.09$ & $2.91\pm0.09$ \\
    $I_{\rm S}$ & $17.98\pm0.12$& $18.72\pm0.09$& $18.90\pm0.07$& $19.21\pm0.08$\\
    $(V-I)_{\rm S,0}$ & $1.03\pm0.11$ & $0.96\pm0.09$& $0.95\pm0.09$& $0.95\pm0.09$\\
    $I_{\rm S,0}$ & $15.55\pm0.13$& $16.29\pm0.10$& $16.48\pm0.09$& $16.78\pm0.09$\\
    $\theta_\ast$ ($\mu$as)& $3.587\pm0.689$& $2.420\pm0.418$& $2.206\pm0.374$& $1.909\pm0.328$\\
    $\theta_{\rm E}$ (mas)& $>0.206$& $>0.236$& $>0.387$& $>0.374$\\
    $\mu_{\rm rel}$ (mas $\mathrm{yr}^{-1}$)& $>3.25$& $>3.74$& $>6.15$& $>5.92$\\
    \hline
    \end{tabular}
    %\tablecomments{$P_\mathrm{{bulge}}$ is the probability that the lens is in the Galactic bulge.}
    \label{lens2}
\end{table*}
